FRL-FI: Transient Fault Analysis for Federated Reinforcement Learning-Based Navigation Systems

Swarm intelligence is being increasingly deployed in autonomous systems, such as drones and unmanned vehicles. Federated reinforcement learning (FRL), a key swarm intelligence paradigm where agents interact with their own environments and cooperatively learn a consensus policy while preserving privacy, has recently shown potential advantages and gained popularity. However, transient faults are increasing in the hardware system with continuous technology node scaling and can pose threats to FRL systems. Meanwhile, conventional redundancy-based protection methods are challenging to deploy on resource-constrained edge applications. In this paper, we experimentally evaluate the fault tolerance of FRL navigation systems at various scales with respect to fault models, fault locations, learning algorithms, layer types, communication intervals, and data types at both training and inference stages. We further propose two cost-effective fault detection and recovery techniques that can achieve up to 3.3x improvement in resilience with <2.7% overhead in FRL systems.

==> tabs/FI_comp.tex <==
\begin{table}[t!]
\centering
\vspace{-5pt}
\caption{Comparison of fault injection techniques at various layers of abstraction. Software-level approach is adopted in our experiments.}
\vspace{-3pt}
\renewcommand*{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{Abstraction}\\ \textbf{Layer} \end{tabular} & \textbf{Platform}                                                                 & \begin{tabular}[c]{@{}c@{}}\textbf{Perf.}\\ \textbf{(cycles/sec)} \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Drone E2E Exec.}\\ \textbf{Time (1 run)} \end{tabular}  & \begin{tabular}[c]{@{}c@{}}\textbf{Drone E2E Exec.}\\ \textbf{Time (1000 runs)} \end{tabular} \\ \hline

RTL                  & \begin{tabular}[c]{@{}c@{}}IVM processor\\ RTL simulation~\cite{maniatakos2010instruction} \end{tabular} & 6$\times$$10^2$     & 2.5$\times$$10^{5}$ hours               & 1.04$\times$$10^{7}$days                 \\ \hline 

Micro-architecture         & gem5 simulator~\cite{binkert2011gem5}                                                                    & 3$\times$$10^6$     & 50.0 hours                 & 2083 days                    \\ \hline
\begin{tabular}[c]{@{}c@{}}FPGA Emulation \end{tabular}   & \begin{tabular}[c]{@{}c@{}}OpenSPARC T1\\ FPGA emulation~\cite{pellegrini2012crashtest} \end{tabular}                                                     & 1$\times$$10^7$     & 15 hours                   & 624 days                     \\ \hline

Architecture               & TSIM simulator~\cite{danvek2013leon3}                                                              & 6$\times$$10^7$     & 2.50 hours                 & 104.2 days                    \\ \hline



\textbf{Software (Ours)}            & \textbf{CPU processor} ~\cite{yim2010measurement}                                                                     & \textbf{3$\mathbf{\times 10^9}$}     & \textbf{3 mins}                     & \textbf{2.09 days}                    \\ \hline

\end{tabular}
}
\label{tab:FI_compare}
\vspace{-5pt}
\end{table}

